Dynamics of the spiral-arm corotation and its observable footprints in the Solar Neighborhood

This article discusses the effects of the spiral-arm corotation on the stellar dynamics in the Solar Neighborhood (SN). All our results presented here rely on: 1) observational evidence that the Sun lies near the corotation circle, where stars rotate with the same angular velocity as the spiral-arm pattern; the corotation circle establishes domains of the corotation resonance (CR) in the Galactic disk; 2) dynamical constraints that put the spiral-arm potential as the dominant perturbation in the SN, comparing with the effects of the central bar in the SN; 3) a long-lived nature of the spiral structure, promoting a state of dynamical relaxing and phase-mixing of the stellar orbits in response to the spiral perturbation. With an analytical model for the Galactic potential, composed of an axisymmetric background deduced from the observed rotation curve, and perturbed by a four-armed spiral pattern, numerical simulations of stellar orbits are performed to delineate the domains of regular and chaotic motions shaped by the resonances. Such studies show that stars can be trapped inside the stable zones of the spiral CR, and this orbital trapping mechanism could explain the dynamical origin of the Local arm of the Milky Way (MW). The spiral CR and the near high-order epicyclic resonances influence the velocity distribution in the SN, creating the observable structures such as moving groups and their radially extended counterpart known as diagonal ridges. The Sun and most of the SN stars evolve inside a stable zone of the spiral CR, never crossing the main spiral-arm structure, but oscillating in the region between the Sagittarius-Carina and Perseus arms. This orbital behavior of the Sun brings insights to our understanding of questions concerning the solar system evolution, the Earth environment changes, and the preservation of life on Earth.

==> refs.tex <==
@ARTICLE{GaiaEDR3,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M.},
        title = "{Gaia Early Data Release 3: Summary of the contents and survey properties}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.01533},
        pages = {arXiv:2012.01533},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201201533G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antoja2008,
       author = {{Antoja}, T. and {Figueras}, F. and {Fern{\'a}ndez}, D. and {Torra}, J.},
        title = "{Origin and evolution of moving groups. I. Characterization in the observational kinematic-age-metallicity space}",
      journal = {A\&A},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: solar neighbourhood, stars: kinematics, methods: data analysis, Astrophysics},
         year = 2008,
        month = oct,
       volume = {490},
       number = {1},
        pages = {135-150},
          doi = {10.1051/0004-6361:200809519},
archivePrefix = {arXiv},
       eprint = {0809.0511},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...490..135A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Eggen1996,
       author = {{Eggen}, Olin J.},
        title = "{Star Streams and Galactic Structure}",
      journal = {AJ},
     keywords = {GALAXY STRUCTURE, GALAXY: KINEMATICS AND DYNAMICS},
         year = 1996,
        month = oct,
       volume = {112},
        pages = {1595},
          doi = {10.1086/118126},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996AJ....112.1595E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SB2002,
       author = {{Sellwood}, J.~A. and {Binney}, J.~J.},
        title = "{Radial mixing in galactic discs}",
      journal = {MNRAS},
     keywords = {ISM: abundances, Galaxy: abundances, Galaxy: kinematics and dynamics, galaxies: evolution, galaxies: ISM, galaxies: structure, Astrophysics},
         year = 2002,
        month = nov,
       volume = {336},
       number = {3},
        pages = {785-796},
          doi = {10.1046/j.1365-8711.2002.05806.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0203510},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.336..785S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Malkin2013,
       author = {{Malkin}, Zinovy},
        title = "{Statistical analysis of the determinations of the Sun's Galactocentric distance}",
     keywords = {Galaxy: center, Galaxy: fundamental parameters, Astrophysics - Galaxy Astrophysics},
    booktitle = {Advancing the Physics of Cosmic Distances},
         year = 2013,
       editor = {{de Grijs}, Richard},
       volume = {289},
        month = feb,
        pages = {406-409},
          doi = {10.1017/S1743921312021825},
archivePrefix = {arXiv},
       eprint = {1306.5519},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013IAUS..289..406M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Honig15,
       author = {{Honig}, Z.~N. and {Reid}, M.~J.},
        title = "{Characteristics of Spiral Arms in Late-type Galaxies}",
      journal = {ApJ},
     keywords = {galaxies: individual: M51 M74 NGC 1232 NGC 3184, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {800},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.1088/0004-637X/800/1/53},
archivePrefix = {arXiv},
       eprint = {1412.1012},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...800...53H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vandeHulst54,
       author = {{van de Hulst}, H.~C. and {Muller}, C.~A. and {Oort}, J.~H.},
        title = "{The spiral structure of the outer part of the Galactic System derived from the hydrogen emission at 21 cm wavelength}",
      journal = {
    Bulletin of the Astronomical Institutes of the Netherlands},
         year = 1954,
        month = may,
       volume = {12},
        pages = {117},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1954BAN....12..117V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{OortMuller52,
       author = {{Oort}, J.~H. and {Muller}, C.~A.},
        title = "{Spiral Structure and Interstellar Emission}",
      journal = {Monthly Notes of the Astronomical Society of South Africa},
     keywords = {galaxies: general, techniques: radio astronomy},
         year = 1952,
        month = jan,
       volume = {11},
        pages = {65},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1952MNSSA..11...65O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Morgan53,
       author = {{Morgan}, W.~W. and {Whitford}, A.~E. and {Code}, A.~D.},
        title = "{Studies in Galactic Structure. I. a Preliminary Determination of the Space Distribution of the Blue Giants.}",
      journal = {ApJ},
         year = 1953,
        month = sep,
       volume = {118},
        pages = {318},
          doi = {10.1086/145754},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1953ApJ...118..318M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Burton_Gordon1978,
   author = {{Burton}, W.~B. and {Gordon}, M.~A.},
    title = "{Carbon monoxide in the Galaxy. III - The overall nature of its distribution in the equatorial plane}",
  journal = {A\&A},
 keywords = {CARBON MONOXIDE, GALACTIC NUCLEI, GALACTIC RADIATION, HYDROGEN CLOUDS, INTERSTELLAR GAS, MOLECULAR ROTATION, ABUNDANCE, ASTRONOMICAL MODELS, EMISSION SPECTRA, HYDROGEN ATOMS, MOLECULAR SPECTRA, STOCHASTIC PROCESSES},
     year = 1978,
    month = feb,
   volume = 63,
    pages = {7-27},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26A....63....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clemens1985,
   author = {{Clemens}, D.~P.},
    title = "{Massachusetts-Stony Brook Galactic plane CO survey - The Galactic disk rotation curve}",
  journal = {ApJ},
 keywords = {CARBON MONOXIDE, GALACTIC ROTATION, INTERSTELLAR GAS, MILKY WAY GALAXY, ANGULAR VELOCITY, GALACTIC NUCLEI, H II REGIONS, RADIAL VELOCITY},
     year = 1985,
    month = aug,
   volume = 295,
    pages = {422-428},
      doi = {10.1086/163386},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...295..422C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fich_Blitz_Stark1989,
   author = {{Fich}, M. and {Blitz}, L. and {Stark}, A.~A.},
    title = "{The rotation curve of the Milky Way to 2 R(0)}",
  journal = {ApJ},
 keywords = {GALACTIC ROTATION, MILKY WAY GALAXY, SPECTROPHOTOMETRY, CARBON MONOXIDE, ERROR ANALYSIS, H II REGIONS, NORTHERN SKY, PLANETARY NEBULAE},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {272-284},
      doi = {10.1086/167591},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342..272F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid_etal2014,
   author = {{Reid}, M.~J. and {Menten}, K.~M. and {Brunthaler}, A. and {Zheng}, X.~W. and
	{Dame}, T.~M. and {Xu}, Y. and {Wu}, Y. and {Zhang}, B. and
	{Sanna}, A. and {Sato}, M. and {Hachisuka}, K. and {Choi}, Y.~K. and
	{Immer}, K. and {Moscadelli}, L. and {Rygl}, K.~L.~J. and {Bartkiewicz}, A.
	},
    title = "{Trigonometric Parallaxes of High Mass Star Forming Regions: The Structure and Kinematics of the Milky Way}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1401.5377},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure, gravitational waves, parallaxes, stars: formation},
     year = 2014,
    month = mar,
   volume = 783,
      eid = {130},
    pages = {130},
      doi = {10.1088/0004-637X/783/2/130},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...783..130R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rastorguev_etal2017,
       author = {{Rastorguev}, A.~S. and {Utkin}, N.~D. and {Zabolotskikh}, M.~V. and
         {Dambis}, A.~K. and {Bajkova}, A.~T. and {Bobylev}, V.~V.},
        title = "{Galactic masers: Kinematics, spiral structure and the disk dynamic state}",
      journal = {Astrophysical Bulletin},
     keywords = {Astrophysics - Astrophysics of Galaxies, 85A05, J.2},
         year = 2017,
        month = apr,
       volume = {72},
       number = {2},
        pages = {122-140},
          doi = {10.1134/S1990341317020043},
archivePrefix = {arXiv},
       eprint = {1603.09124},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AstBu..72..122R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid_Brunthaler2004,
   author = {{Reid}, M.~J. and {Brunthaler}, A.},
    title = "{The Proper Motion of Sagittarius A*. II. The Mass of Sagittarius A*}",
  journal = {ApJ},
   eprint = {arXiv:astro-ph/0408107},
 keywords = {Astrometry, Black Hole Physics, Galaxy: Center, Galaxy: Fundamental Parameters, Galaxy: Structure},
     year = 2004,
    month = dec,
   volume = 616,
    pages = {872-884},
      doi = {10.1086/424960},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616..872R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schonrich_etal2010,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J. and {Dehnen}, W.},
    title = "{Local kinematics and the local standard of rest}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {0912.3693},
 primaryClass = "astro-ph.GA",
 keywords = {stars: kinematics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, solar neighbourhood},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {1829-1833},
      doi = {10.1111/j.1365-2966.2010.16253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403.1829S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allen_Santillan1991,
   author = {{Allen}, C. and {Santillan}, A.},
    title = "{An improved model of the galactic mass distribution for orbit computations}",
  journal = {Rev. Mexicana Astron. Astrofis.},
 keywords = {Astronomical Models, Galactic Mass, Mass Distribution, Milky Way Galaxy, Stellar Motions, Dynamic Models, Galactic Rotation, Galactic Structure, Mathematical Models},
     year = 1991,
    month = oct,
   volume = 22,
    pages = {255-263},
   adsurl = {http://adsabs.harvard.edu/abs/1991RMxAA..22..255A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Irrgang2013,
   author = {{Irrgang}, A. and {Wilcox}, B. and {Tucker}, E. and {Schiefelbein}, L.
	},
    title = "{Milky Way mass models for orbit calculations}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1211.4353},
 primaryClass = "astro-ph.GA",
 keywords = {dark matter, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: kinematics and dynamics},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A137},
    pages = {A137},
      doi = {10.1051/0004-6361/201220540},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A.137I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barros_etal2016,
       author = {{Barros}, D.~A. and {L{\'e}pine}, J.~R.~D. and {Dias}, W.~S.},
        title = "{Models for the 3D axisymmetric gravitational potential of the Milky Way galaxy. A detailed modelling of the Galactic disk}",
      journal = {A\&A},
     keywords = {Galaxy: disk, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure, methods: numerical, methods: statistical, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = sep,
       volume = {593},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/201527535},
archivePrefix = {arXiv},
       eprint = {1607.02541},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...593A.108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dehnen_Binney1998,
   author = {{Dehnen}, W. and {Binney}, J.},
    title = "{Mass models of the Milky Way}",
  journal = {MNRAS},
   eprint = {astro-ph/9612059},
 keywords = {Milky Way Galaxy, Galactic Mass, Astronomical Models, Galactic Structure, Mass Distribution, Galactic Halos, Luminosity, Density Distribution},
     year = 1998,
    month = mar,
   volume = 294,
    pages = {429},
      doi = {10.1046/j.1365-8711.1998.01282.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.294..429D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McMillan2011,
   author = {{McMillan}, P.~J.},
    title = "{Mass models of the Milky Way}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1102.4340},
 primaryClass = "astro-ph.GA",
 keywords = {methods: statistical, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2446-2457},
      doi = {10.1111/j.1365-2966.2011.18564.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2446M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Georgelin_Georgelin1976,
   author = {{Georgelin}, Y.~M. and {Georgelin}, Y.~P.},
    title = "{The spiral structure of our Galaxy determined from H II regions}",
  journal = {A\&A},
 keywords = {ASTRONOMICAL MODELS, GALACTIC ROTATION, GALACTIC STRUCTURE, H ALPHA LINE, H II REGIONS, MILKY WAY GALAXY, ASTRONOMICAL MAPS, HYDROGEN IONS, KINEMATICS, RADIAL VELOCITY, RADIO ASTRONOMY, TABLES (DATA), VISUAL OBSERVATION},
     year = 1976,
    month = may,
   volume = 49,
    pages = {57-79},
   adsurl = {http://adsabs.harvard.edu/abs/1976A%26A....49...57G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Russeil2003,
   author = {{Russeil}, D.},
    title = "{Star-forming complexes and the spiral structure of our Galaxy}",
  journal = {A\&A},
 keywords = {ISM: HII regions, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2003,
    month = jan,
   volume = 397,
    pages = {133-146},
      doi = {10.1051/0004-6361:20021504},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...397..133R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Paladini2004,
   author = {{Paladini}, R. and {Davies}, R.~D. and {De Zotti}, G.},
    title = "{Spatial distribution of Galactic HII regions}",
  journal = {MNRAS},
   eprint = {arXiv:astro-ph/0309350},
 keywords = {HII regions, Galaxy: structure, radio continuum: ISM},
     year = 2004,
    month = jan,
   volume = 347,
    pages = {237-245},
      doi = {10.1111/j.1365-2966.2004.07210.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.347..237P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Efremov2011,
   author = {{Efremov}, Y.~N.},
    title = "{On the spiral structure of the Milky Way Galaxy}",
  journal = {Astron. Rep.},
archivePrefix = "arXiv",
   eprint = {1011.4576},
 primaryClass = "astro-ph.CO",
     year = 2011,
    month = feb,
   volume = 55,
    pages = {108-122},
      doi = {10.1134/S1063772911020016},
   adsurl = {http://adsabs.harvard.edu/abs/2011ARep...55..108E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hou_Han2014,
   author = {{Hou}, L.~G. and {Han}, J.~L.},
    title = "{The observed spiral structure of the Milky Way}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1407.7331},
 keywords = {Galaxy: disk, Galaxy: structure, Galaxy: kinematics and dynamics, HII regions, ISM: clouds},
     year = 2014,
    month = sep,
   volume = 569,
      eid = {A125},
    pages = {A125},
      doi = {10.1051/0004-6361/201424039},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...569A.125H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ortiz_Lepine1993,
   author = {{Ortiz}, R. and {Lepine}, J.~R.~D.},
    title = "{A model of the Galaxy for predicting star counts in the infrared}",
  journal = {A\&A},
 keywords = {ASTRONOMICAL MODELS, GALACTIC STRUCTURE, INFRARED ASTRONOMY, INFRARED STARS, MATHEMATICAL MODELS, MILKY WAY GALAXY, STAR DISTRIBUTION, COSMIC DUST, DISKS (SHAPES), INFRARED ASTRONOMY SATELLITE, INTERSTELLAR EXTINCTION, INTERSTELLAR MATTER, STELLAR ENVELOPES, STELLAR LUMINOSITY, STELLAR MAGNITUDE},
     year = 1993,
    month = nov,
   volume = 279,
    pages = {90-106},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...279...90O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Drimmel_Spergel2001,
   author = {{Drimmel}, R. and {Spergel}, D.~N.},
    title = "{Three-dimensional Structure of the Milky Way Disk: The Distribution of Stars and Dust beyond 0.35 R$_{solar}$}",
  journal = {ApJ},
   eprint = {arXiv:astro-ph/0101259},
 keywords = {ISM: Dust, Extinction, Galaxy: Disk, Galaxy: Disk, Galaxy: Structure, Infrared: Stars, Infrared: ISM},
     year = 2001,
    month = jul,
   volume = 556,
    pages = {181-202},
      doi = {10.1086/321556},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..181D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Churchwell2009,
   author = {{Churchwell}, E. and {Babler}, B.~L. and {Meade}, M.~R. and 
	{Whitney}, B.~A. and {Benjamin}, R. and {Indebetouw}, R. and 
	{Cyganowski}, C. and {Robitaille}, T.~P. and {Povich}, M. and 
	{Watson}, C. and {Bracker}, S.},
    title = "{The Spitzer/GLIMPSE Surveys: A New View of the Milky Way}",
  journal = {PASP},
 keywords = {IYA Review},
     year = 2009,
    month = mar,
   volume = 121,
    pages = {213-230},
      doi = {10.1086/597811},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASP..121..213C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine2011a,
   author = {{L{\'e}pine}, J.~R.~D. and {Roman-Lopes}, A. and {Abraham}, Z. and 
	{Junqueira}, T.~C. and {Mishurov}, Y.~N.},
    title = "{The spiral structure of the Galaxy revealed by CS sources and evidence for the 4:1 resonance}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1010.1790},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = {2011a},
    month = jun,
   volume = 414,
    pages = {1607-1616},
      doi = {10.1111/j.1365-2966.2011.18492.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.1607L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chernin1999,
   author = {{Chernin}, A.~D.},
    title = "{Spiral patterns with straight arm segments}",
  journal = {MNRAS},
     year = 1999,
    month = sep,
   volume = 308,
    pages = {321-332},
      doi = {10.1046/j.1365-8711.1999.02585.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..321C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antoja2011,
   author = {{Antoja}, T. and {Figueras}, F. and {Romero-G{\'o}mez}, M. and 
	{Pichardo}, B. and {Valenzuela}, O. and {Moreno}, E.},
    title = "{Understanding the spiral structure of the Milky Way using the local kinematic groups}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1106.1170},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, Galaxy: evolution, Galaxy: kinematics and dynamics, solar neighbourhood, Galaxy: structure, galaxies: spiral},
     year = 2011,
    month = dec,
   volume = 418,
    pages = {1423-1440},
      doi = {10.1111/j.1365-2966.2011.19190.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418.1423A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vallee2016,
       author = {{Vall{\'e}e}, Jacques P.},
        title = "{The Start of the Sagittarius Spiral Arm (Sagittarius Origin) and the Start of the Norma Spiral Arm (Norma Origin): Model-computed and Observed Arm Tangents at Galactic Longitudes -20$^{\circ}$ $<$ l $<$ +23$^{\circ}$}",
      journal = {AJ},
     keywords = {galaxies: spiral, Galaxy: disk, Galaxy: structure, ISM: general, ISM: structure, methods: statistical, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = mar,
       volume = {151},
       number = {3},
          eid = {55},
        pages = {55},
          doi = {10.3847/0004-6256/151/3/55},
archivePrefix = {arXiv},
       eprint = {1602.02183},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016AJ....151...55V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vallee2015,
       author = {{Vall{\'e}e}, Jacques P.},
        title = "{Different studies of the global pitch angle of the Milky Way's spiral arms}",
      journal = {MNRAS},
     keywords = {methods: statistical, ISM: general, ISM: structure, Galaxy: disc, Galaxy: structure, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {450},
       number = {4},
        pages = {4277-4284},
          doi = {10.1093/mnras/stv862},
archivePrefix = {arXiv},
       eprint = {1505.01202},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.4277V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bobylev_Bajkova2013,
       author = {{Bobylev}, V.~V. and {Bajkova}, A.~T.},
        title = "{Estimation of the pitch angle of the Galactic spiral pattern}",
      journal = {Astronomy Letters},
     keywords = {Galactic structure, outer arm, spiral density waves, masers, open star clusters},
         year = 2013,
        month = nov,
       volume = {39},
       number = {11},
        pages = {759-764},
          doi = {10.1134/S1063773713110017},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013AstL...39..759B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine_etal2017,
       author = {{L{\'e}pine}, Jacques R.~D. and {Michtchenko}, Tatiana A. and
         {Barros}, Douglas A. and {Vieira}, Ronaldo S.~S.},
        title = "{The Dynamical Origin of the Local Arm and the Sun's Trapped Orbit}",
      journal = {ApJ},
     keywords = {Galaxy: disk, kinematics and dynamics, solar neighborhood, structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {843},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.3847/1538-4357/aa72e5},
archivePrefix = {arXiv},
       eprint = {1705.04381},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843...48L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lin_Shu1964,
   author = {{Lin}, C.~C. and {Shu}, F.~H.},
    title = "{On the Spiral Structure of Disk Galaxies.}",
  journal = {ApJ},
     year = 1964,
    month = aug,
   volume = 140,
    pages = {646},
      doi = {10.1086/147955},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...140..646L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Binney_Tremaine2008,
   author = {{Binney}, J. and {Tremaine}, S.},
    title = "{Galactic Dynamics: Second Edition}",
booktitle = {Galactic Dynamics: Second Edition, by James Binney and Scott Tremaine.~ISBN 978-0-691-13026-2 (HB).~Published by Princeton University Press, Princeton, NJ USA, 2008.},
     year = 2008,
publisher = {Princeton University Press},
   adsurl = {http://adsabs.harvard.edu/abs/2008gady.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalnajs1973,
   author = {{Kalnajs}, A.~J.},
    title = "{Spiral Structure Viewed as a Density Wave}",
  journal = {PASAu},
     year = 1973,
    month = oct,
   volume = 2,
    pages = {174},
   adsurl = {http://adsabs.harvard.edu/abs/1973PASAu...2..174K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Contopoulos_Grosbol1986,
   author = {{Contopoulos}, G. and {Grosbol}, P.},
    title = "{Stellar dynamics of spiral galaxies - Nonlinear effects at the 4/1 resonance}",
  journal = {A\&A},
 keywords = {ASTRONOMICAL MODELS, RESONANCE, SPIRAL GALAXIES, STELLAR ORBITS, COROTATION, DENSITY DISTRIBUTION, INTERSTELLAR GAS, NONLINEAR SYSTEMS},
     year = 1986,
    month = jan,
   volume = 155,
    pages = {11-23},
   adsurl = {http://adsabs.harvard.edu/abs/1986A%26A...155...11C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Contopoulos_Grosbol1988,
       author = {{Contopoulos}, G. and {Grosbol}, P.},
        title = "{Stellar dynamics of spiral galaxies : self-consistent models.}",
      journal = {A\&A},
     keywords = {Astrodynamics, Astronomical Models, Barred Galaxies, Molecular Clouds, Spiral Galaxies, Stellar Motions, Computational Astrophysics, Corotation, Self Consistent Fields, Astrophysics},
         year = 1988,
        month = may,
       volume = {197},
        pages = {83-90},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&A...197...83C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patsis1991,
   author = {{Patsis}, P.~A. and {Contopoulos}, G. and {Grosbol}, P.},
    title = "{Self-consistent spiral galactic models}",
  journal = {A\&A},
 keywords = {ASTRONOMICAL MODELS, GALACTIC STRUCTURE, SELF CONSISTENT FIELDS, SPIRAL GALAXIES, ASTRONOMICAL PHOTOMETRY, GALACTIC ROTATION, PERTURBATION THEORY},
     year = 1991,
    month = mar,
   volume = 243,
    pages = {373-380},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...243..373P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amaral_Lepine1997,
   author = {{Amaral}, L.~H. and {Lepine}, J.~R.~D.},
    title = "{A self-consistent model of the spiral structure of the Galaxy}",
  journal = {MNRAS},
 keywords = {GALAXY: KINEMATICS AND DYNAMICS, GALAXY: STRUCTURE},
     year = 1997,
    month = apr,
   volume = 286,
    pages = {885-894},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.286..885A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pichardo2003,
   author = {{Pichardo}, B. and {Martos}, M. and {Moreno}, E. and {Espresate}, J.
	},
    title = "{Nonlinear Effects in Models of the Galaxy. I. Midplane Stellar Orbits in the Presence of Three-dimensional Spiral Arms}",
  journal = {ApJ},
   eprint = {arXiv:astro-ph/0208136},
 keywords = {Galaxies: Kinematics and Dynamics, Galaxy: Kinematics and Dynamics, Galaxy: Structure, Magnetohydrodynamics: MHD, Shock Waves, Stellar Dynamics},
     year = 2003,
    month = jan,
   volume = 582,
    pages = {230-245},
      doi = {10.1086/344592},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...582..230P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Junqueira2013,
   author = {{Junqueira}, T.~C. and {L{\'e}pine}, J.~R.~D. and {Braga}, C.~A.~S. and 
	{Barros}, D.~A.},
    title = "{A new model for gravitational potential perturbations in disks of spiral galaxies. An application to our Galaxy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1212.3312},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: spiral, galaxies: bulges},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A91},
    pages = {A91 (JLBB)},
      doi = {10.1051/0004-6361/201219769},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A..91J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Michtchenko_etal2017,
       author = {{Michtchenko}, T.~A. and {Vieira}, R.~S.~S. and {Barros}, D.~A. and
         {L{\'e}pine}, J.~R.~D.},
        title = "{Modelling resonances and orbital chaos in disk galaxies. Application to a Milky Way spiral model}",
      journal = {A\&A},
     keywords = {galaxies: spiral, Galaxy: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Nonlinear Sciences - Chaotic Dynamics},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A39},
        pages = {A39},
          doi = {10.1051/0004-6361/201628895},
archivePrefix = {arXiv},
       eprint = {1608.08991},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A..39M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Michtchenko_etal2018a,
       author = {{Michtchenko}, T.~A. and {L{\'e}pine}, J.~R.~D. and {Barros}, D.~A. and
         {Vieira}, R.~S.~S.},
        title = "{Combined dynamical effects of the bar and spiral arms in a Galaxy model. Application to the solar neighbourhood}",
      journal = {A\&A},
     keywords = {galaxies: spiral, Galaxy: kinematics and dynamics, solar neighborhood, methods: analytical, methods: numerical, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jul,
       volume = {615},
          eid = {A10},
        pages = {A10},
          doi = {10.1051/0004-6361/201833035},
archivePrefix = {arXiv},
       eprint = {1803.06995},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...615A..10M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Ferraz-Mello2007,
       author = {{Ferraz-Mello}, Sylvio},
        title = "{Canonical Perturbation Theories - Degenerate Systems and Resonance}",
         year = 2007,
    publisher = {Astrophysics and Space Science Library, Springer US},
       volume = {345},
          doi = {10.1007/978-0-387-38905-9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ASSL..345.....F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lynden-Bell_Kalnajs1972,
   author = {{Lynden-Bell}, D. and {Kalnajs}, A.~J.},
    title = "{On the generating mechanism of spiral structure}",
  journal = {MNRAS},
     year = 1972,
   volume = 157,
    pages = {1},
   adsurl = {http://adsabs.harvard.edu/abs/1972MNRAS.157....1L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Xu_etal2016,
       author = {{Xu}, Y. and {Reid}, M. and {Dame}, T. and {Menten}, K. and {Sakai}, N. and
         {Li}, J. and {Brunthaler}, A. and {Moscadelli}, L. and {Zhang}, B. and
         {Zheng}, X.},
        title = "{The local spiral structure of the Milky Way}",
      journal = {Science Advances},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = sep,
       volume = {2},
       number = {9},
        pages = {e1600878-e1600878},
          doi = {10.1126/sciadv.1600878},
archivePrefix = {arXiv},
       eprint = {1610.00242},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SciA....2E0878X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Murray_Dermott1999,
       author = {{Murray}, C.~D. and {Dermott}, S.~F.},
        title = "{Solar system dynamics}",
         year = 1999,
    publisher = {Cambridge, UK: Cambridge University Press},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ssd..book.....M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{contopoulos1973ApJ,
  author = {{Contopoulos}, G.},
  title = {{The Particle Resonance in Spiral Galaxies. Nonlinear Effects}},
  journal = {ApJ},
  year = {1973},
  volume = {181},
  pages = {657-684},
  month = may,
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  doi = {10.1086/152080},
  url = {http://adsabs.harvard.edu/abs/1973ApJ...181..657C}
}

@ARTICLE{barbanis1976AA,
  author = {{Barbanis}, B.},
  title = {{Density Maxima Formed by Trapped Orbits}},
  journal = {A\&A},
  year = {1976},
  volume = {46},
  pages = {269},
  month = jan,
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl = {http://adsabs.harvard.edu/abs/1976A%26A....46..269B}
}

@ARTICLE{gomezEtal2013MNRAS,
  author = {{G{\'o}mez}, G.~C. and {Pichardo}, B. and {Martos}, M.~A.},
  title = {{Comparing gaseous and stellar orbits in a spiral potential}},
  journal = {MNRAS},
  year = {2013},
  volume = {430},
  pages = {3010-3016},
  month = apr,
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430.3010G},
  archiveprefix = {arXiv},
  doi = {10.1093/mnras/stt107},
  eprint = {1301.4284},
  keywords = {MHD, Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: structure,
	galaxies: spiral, galaxies: structure}
}

@ARTICLE{liEtal2016ApJ,
  author = {{Li}, Z. and {Gerhard}, O. and {Shen}, J. and {Portail}, M. and {Wegg},
	C.},
  title = {{Gas Dynamics in the Milky Way: A Low Pattern Speed Model}},
  journal = {ApJ},
  year = {2016},
  volume = {824},
  pages = {13},
  month = jun,
  eid = {13},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...824...13L},
  archiveprefix = {arXiv},
  doi = {10.3847/0004-637X/824/1/13},
  eprint = {1603.09650},
  keywords = {galaxies: ISM, galaxies: kinematics and dynamics, galaxies: structure,
	hydrodynamics}
}

@ARTICLE{Dehnen2000,
       author = {{Dehnen}, Walter},
        title = "{The Effect of the Outer Lindblad Resonance of the Galactic Bar on the Local Stellar Velocity Distribution}",
      journal = {AJ},
     keywords = {GALAXY: KINEMATICS AND DYNAMICS, GALAXY: STRUCTURE, GALAXY: SOLAR NEIGHBORHOOD, Astrophysics},
         year = 2000,
        month = feb,
       volume = {119},
       number = {2},
        pages = {800-812},
          doi = {10.1086/301226},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911161},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000AJ....119..800D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Minchev_etal2007,
       author = {{Minchev}, I. and {Nordhaus}, J. and {Quillen}, A.~C.},
        title = "{New Constraints on the Galactic Bar}",
      journal = {ApJL},
     keywords = {Galaxy: Fundamental Parameters, Galaxy: Kinematics and Dynamics, Galaxy: Structure, Galaxy: Solar Neighborhood, Astrophysics},
         year = 2007,
        month = jul,
       volume = {664},
       number = {1},
        pages = {L31-L34},
          doi = {10.1086/520578},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703805},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...664L..31M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antoja_etal2014,
       author = {{Antoja}, T. and {Helmi}, A. and {Dehnen}, W. and {Bienaym{\'e}}, O. and
         {Bland-Hawthorn}, J. and {Famaey}, B. and {Freeman}, K. and
         {Gibson}, B.~K. and {Gilmore}, G. and {Grebel}, E.~K. and
         {Kordopatis}, G. and {Kunder}, A. and {Minchev}, I. and {Munari}, U. and
         {Navarro}, J. and {Parker}, Q. and {Reid}, W.~A. and {Seabroke}, G. and
         {Siebert}, A. and {Steinmetz}, M. and {Watson}, F. and
         {Wyse}, R.~F.~G. and {Zwitter}, T.},
        title = "{Constraints on the Galactic bar from the Hercules stream as traced with RAVE across the Galaxy}",
      journal = {A\&A},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, Galaxy: disk, Galaxy: evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = mar,
       volume = {563},
          eid = {A60},
        pages = {A60},
          doi = {10.1051/0004-6361/201322623},
archivePrefix = {arXiv},
       eprint = {1309.4272},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...563A..60A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perez-Villegas_etal2017,
       author = {{P{\'e}rez-Villegas}, Angeles and {Portail}, Matthieu and
         {Wegg}, Christopher and {Gerhard}, Ortwin},
        title = "{Revisiting the Tale of Hercules: How Stars Orbiting the Lagrange Points Visit the Sun}",
      journal = {ApJL},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, solar neighborhood, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = may,
       volume = {840},
       number = {1},
          eid = {L2},
        pages = {L2},
          doi = {10.3847/2041-8213/aa6c26},
archivePrefix = {arXiv},
       eprint = {1702.06541},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...840L...2P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antoja_etal2011,
       author = {{Antoja}, T. and {Figueras}, F. and {Romero-G{\'o}mez}, M. and
         {Pichardo}, B. and {Valenzuela}, O. and {Moreno}, E.},
        title = "{Understanding the spiral structure of the Milky Way using the local kinematic groups}",
      journal = {MNRAS},
     keywords = {Galaxy: disc, Galaxy: evolution, Galaxy: kinematics and dynamics, solar neighbourhood, Galaxy: structure, galaxies: spiral, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {418},
       number = {3},
        pages = {1423-1440},
          doi = {10.1111/j.1365-2966.2011.19190.x},
archivePrefix = {arXiv},
       eprint = {1106.1170},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.418.1423A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quillen_etal2018,
       author = {{Quillen}, Alice C. and {Carrillo}, Ismael and {Anders}, Friedrich and
         {McMillan}, Paul and {Hilmi}, Tariq and {Monari}, Giacomo and
         {Minchev}, Ivan and {Chiappini}, Cristina and {Khalatyan}, Arman and
         {Steinmetz}, Matthias},
        title = "{Spiral arm crossings inferred from ridges in Gaia stellar velocity distributions}",
      journal = {MNRAS},
     keywords = {Galaxy: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = nov,
       volume = {480},
       number = {3},
        pages = {3132-3139},
          doi = {10.1093/mnras/sty2077},
archivePrefix = {arXiv},
       eprint = {1805.10236},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.3132Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hattori_etal2019,
       author = {{Hattori}, Kohei and {Gouda}, Naoteru and {Tagawa}, Hiromichi and
         {Sakai}, Nobuyuki and {Yano}, Taihei and {Baba}, Junichi and
         {Kumamoto}, Jun},
        title = "{Metallicity dependence of the Hercules stream in Gaia/RAVE data - explanation by non-closed orbits}",
      journal = {MNRAS},
     keywords = {Galaxy: disc, (Galaxy:) solar neighbourhood, Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = apr,
       volume = {484},
       number = {4},
        pages = {4540-4562},
          doi = {10.1093/mnras/stz266},
archivePrefix = {arXiv},
       eprint = {1804.01920},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.4540H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Michtchenko_etal2018b,
       author = {{Michtchenko}, Tatiana A. and {L{\'e}pine}, Jacques R.~D. and
         {P{\'e}rez-Villegas}, Angeles and {Vieira}, Ronaldo S.~S. and
         {Barros}, Douglas A.},
        title = "{On the Stellar Velocity Distribution in the Solar Neighborhood in Light of Gaia DR2}",
      journal = {ApJL},
     keywords = {galaxies: spiral, Galaxy: kinematics and dynamics, Galaxy: structure, solar neighborhood, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = aug,
       volume = {863},
       number = {2},
          eid = {L37},
        pages = {L37},
          doi = {10.3847/2041-8213/aad804},
archivePrefix = {arXiv},
       eprint = {1808.01501},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...863L..37M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia_Collaboration2018a,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and
         {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and
         {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and
         {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and
         {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and
         {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and
         {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and
         {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and
         {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and
         {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and
         {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and
         {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and
         {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and
         {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and
         {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and
         {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and
         {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and
         {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and
         {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and
         {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and
         {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and
         {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and
         {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and
         {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and
         {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and
         {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and
         {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and
         {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and
         {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and
         {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and
         {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and
         {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and
         {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and
         {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and
         {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and
         {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and
         {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and
         {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and
         {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and
         {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and
         {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and
         {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and
         {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and
         {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and
         {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and
         {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and
         {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and
         {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and
         {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and
         {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and
         {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and
         {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and
         {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and
         {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and
         {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and
         {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and
         {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and
         {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and
         {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and
         {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and
         {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and
         {De Luise}, F. and {De March}, R. and {de Martino}, D. and
         {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and
         {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and
         {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and
         {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and
         {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and
         {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and
         {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and
         {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and
         {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and
         {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and
         {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and
         {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and
         {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and
         {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and
         {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and
         {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and
         {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and
         {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and
         {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and
         {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and
         {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and
         {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and
         {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and
         {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and
         {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and
         {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and
         {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and
         {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and
         {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and
         {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and
         {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and
         {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and
         {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and
         {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and
         {Marton}, G. and {Mary}, N. and {Massari}, D. and
         {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and
         {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and
         {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and
         {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and
         {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and
         {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and
         {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and
         {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and
         {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and
         {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and
         {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and
         {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and
         {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and
         {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and
         {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and
         {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and
         {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and
         {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and
         {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and
         {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and
         {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and
         {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and
         {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and
         {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and
         {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and
         {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and
         {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and
         {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssand
        ier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and
         {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and
         {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and
         {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and
         {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and
         {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and
         {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and
         {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and
         {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and
         {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and
         {Zwitter}, T.},
        title = "{Gaia Data Release 2. Summary of the contents and survey properties}",
      journal = {A\&A},
     keywords = {catalogs, astrometry, techniques: radial velocities, stars: fundamental parameters, stars: variables: general, minor planets, asteroids: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = aug,
       volume = {616},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201833051},
archivePrefix = {arXiv},
       eprint = {1804.09365},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barros_etal2020
,
       author = {{Barros}, Douglas A. and {P{\'e}rez-Villegas}, Angeles and
         {L{\'e}pine}, Jacques R.~D. and {Michtchenko}, Tatiana A. and
         {Vieira}, Ronaldo S.~S.},
        title = "{Exploring the Origin of Moving Groups and Diagonal Ridges by Simulations of Stellar Orbits and Birthplaces}",
      journal = {ApJ},
     keywords = {Milky Way disk, Milky Way dynamics, Milky Way evolution, Stellar kinematics, Spiral arms, Solar neighborhood, 1050, 1051, 1052, 1608, 1559, 1509, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {75},
        pages = {75},
          doi = {10.3847/1538-4357/ab59d1},
archivePrefix = {arXiv},
       eprint = {1911.08675},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...75B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antoja_etal2018,
       author = {{Antoja}, T. and {Helmi}, A. and {Romero-G{\'o}mez}, M. and {Katz}, D. and
         {Babusiaux}, C. and {Drimmel}, R. and {Evans}, D.~W. and
         {Figueras}, F. and {Poggio}, E. and {Reyl{\'e}}, C. and {Robin}, A.~C. and
         {Seabroke}, G. and {Soubiran}, C.},
        title = "{A dynamically young and perturbed Milky Way disk}",
      journal = {Nature},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = sep,
       volume = {561},
       number = {7723},
        pages = {360-362},
          doi = {10.1038/s41586-018-0510-7},
archivePrefix = {arXiv},
       eprint = {1804.10196},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018Natur.561..360A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bland-Hawthorn_etal2019,
       author = {{Bland-Hawthorn}, Joss and {Sharma}, Sanjib and {Tepper-Garcia}, Thor and
         {Binney}, James and {Freeman}, Ken C. and {Hayden}, Michael R. and
         {Kos}, Janez and {De Silva}, Gayandhi M. and {Ellis}, Simon and
         {Lewis}, Geraint F. and {Asplund}, Martin and {Buder}, Sven and
         {Casey}, Andrew R. and {D'Orazi}, Valentina and {Duong}, Ly and
         {Khanna}, Shourya and {Lin}, Jane and {Lind}, Karin and
         {Martell}, Sarah L. and {Ness}, Melissa K. and {Simpson}, Jeffrey D. and
         {Zucker}, Daniel B. and {Zwitter}, Toma{\v{z}} and {Kafle}, Prajwal R. and
         {Quillen}, Alice C. and {Ting}, Yuan-Sen and {Wyse}, Rosemary F.~G.},
        title = "{The GALAH survey and Gaia DR2: dissecting the stellar disc's phase space by age, action, chemistry, and location}",
      journal = {MNRAS},
     keywords = {astrometry, proper motions, stars: kinematics and dynamics, Galaxy: disc, evolution, structure, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jun,
       volume = {486},
       number = {1},
        pages = {1167-1191},
          doi = {10.1093/mnras/stz217},
archivePrefix = {arXiv},
       eprint = {1809.02658},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.1167B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Laporte_etal2019,
       author = {{Laporte}, Chervin F.~P. and {Minchev}, Ivan and {Johnston}, Kathryn V. and
         {G{\'o}mez}, Facundo A.},
        title = "{Footprints of the Sagittarius dwarf galaxy in the Gaia data set}",
      journal = {MNRAS},
     keywords = {Galaxy: disc, Galaxy: evolution, Galaxy: formation, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {485},
       number = {3},
        pages = {3134-3152},
          doi = {10.1093/mnras/stz583},
archivePrefix = {arXiv},
       eprint = {1808.00451},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.3134L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Khanna_etal2019,
       author = {{Khanna}, Shourya and {Sharma}, Sanjib and {Tepper-Garcia}, Thor and {Bland
        -Hawthorn}, Joss and {Hayden}, Michael and {Asplund}, Martin and
         {Buder}, Sven and {Chen}, Boquan and {De Silva}, Gayandhi M. and
         {Freeman}, Ken C. and {Kos}, Janez and {Lewis}, Geraint F. and
         {Lin}, Jane and {Martell}, Sarah L. and {Simpson}, Jeffrey D. and
         {Nordlander}, Thomas and {Stello}, Dennis and {Ting}, Yuan-Sen and
         {Zucker}, Daniel B. and {Zwitter}, Toma{\v{z}}},
        title = "{The GALAH survey and Gaia DR2: Linking ridges, arches, and vertical waves in the kinematics of the Milky Way}",
      journal = {MNRAS},
     keywords = {methods: numerical, stars: abundances, galaxy: kinematics and dynamics, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {489},
       number = {4},
        pages = {4962-4979},
          doi = {10.1093/mnras/stz2462},
archivePrefix = {arXiv},
       eprint = {1902.10113},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.4962K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Khoperskov_etal2019,
       author = {{Khoperskov}, Sergey and {Di Matteo}, Paola and {Gerhard}, Ortwin and
         {Katz}, David and {Haywood}, Misha and {Combes}, Fran{\c{c}}oise and
         {Berczik}, Peter and {Gomez}, Ana},
        title = "{The echo of the bar buckling: Phase-space spirals in Gaia Data Release 2}",
      journal = {A\&A},
     keywords = {galaxies: evolution, galaxies: kinematics and dynamics, Galaxy: disk, Galaxy: kinematics and dynamics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {L6},
        pages = {L6},
          doi = {10.1051/0004-6361/201834707},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622L...6K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang_etal2020,
       author = {{Wang}, H. -F. and {Huang}, Y. and {Zhang}, H. -W. and
         {L{\'o}pez-Corredoira}, M. and {Cui}, W. -Y. and {Chen}, B. -Q. and
         {Guo}, R. and {Chang}, J.},
        title = "{Diagonal Ridge Pattern of Different Age Populations Found in Gaia-DR2 with LAMOST Main-sequence Turnoff and OB-type Stars}",
      journal = {ApJ},
     keywords = {Milky Way disk, Milky Way dynamics, Milky Way evolution, Milky Way formation, the Milky Way, 1050, 1051, 1052, 1053, 1054, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = oct,
       volume = {902},
       number = {1},
          eid = {70},
        pages = {70},
          doi = {10.3847/1538-4357/abb3c8},
archivePrefix = {arXiv},
       eprint = {2005.14362},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...902...70W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fragkoudi_etal2019,
       author = {{Fragkoudi}, F. and {Katz}, D. and {Trick}, W. and {White}, S.~D.~M. and
         {Di Matteo}, P. and {Sormani}, M.~C. and {Khoperskov}, S. and
         {Haywood}, M. and {Hall{\'e}}, A. and {G{\'o}mez}, A.},
        title = "{On the ridges, undulations, and streams in Gaia DR2: linking the topography of phase space to the orbital structure of an N-body bar}",
      journal = {MNRAS},
     keywords = {galaxies: kinematics and dynamics, Galaxy: disc, Galaxy: evolution, Galaxy: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = sep,
       volume = {488},
       number = {3},
        pages = {3324-3339},
          doi = {10.1093/mnras/stz1875},
archivePrefix = {arXiv},
       eprint = {1901.07568},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.488.3324F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schonrich_Binney2009,
       author = {{Sch{\"o}nrich}, Ralph and {Binney}, James},
        title = "{Chemical evolution with radial mixing}",
      journal = {MNRAS},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: ISM, galaxies: kinematics and dynamics, Galaxy: disc, solar neighbourhood, Astrophysics},
         year = 2009,
        month = jun,
       volume = {396},
       number = {1},
        pages = {203-222},
          doi = {10.1111/j.1365-2966.2009.14750.x},
archivePrefix = {arXiv},
       eprint = {0809.3006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.396..203S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine_etal2011b,
       author = {{L{\'e}pine}, J.~R.~D. and {Cruz}, P. and {Scarano}, S., Jr. and
         {Barros}, D.~A. and {Dias}, W.~S. and {Pomp{\'e}ia}, L. and
         {Andrievsky}, S.~M. and {Carraro}, G. and {Famaey}, B.},
        title = "{Overlapping abundance gradients and azimuthal gradients related to the spiral structure of the Galaxy}",
      journal = {MNRAS},
     keywords = {stars: kinematics and dynamics, Galaxy: abundances, Galaxy: evolution, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = oct,
       volume = {417},
       number = {1},
        pages = {698-708},
          doi = {10.1111/j.1365-2966.2011.19314.x},
archivePrefix = {arXiv},
       eprint = {1106.3137},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.417..698L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Twarog_etal1997,
       author = {{Twarog}, Bruce A. and {Ashman}, Keith M. and
         {Anthony-Twarog}, Barbara J.},
        title = "{Some Revised Observational Constraints on the Formation and Evolution of the Galactic Disk}",
      journal = {AJ},
     keywords = {GALAXY: EVOLUTION, GALAXY: STRUCTURE, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL, Astrophysics},
         year = 1997,
        month = dec,
       volume = {114},
        pages = {2556},
          doi = {10.1086/118667},
archivePrefix = {arXiv},
       eprint = {astro-ph/9709122},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997AJ....114.2556T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andrievsky_etal2004,
       author = {{Andrievsky}, S.~M. and {Luck}, R.~E. and {Martin}, P. and
         {L{\'e}pine}, J.~R.~D.},
        title = "{The Galactic abundance gradient from Cepheids. V. Transition zone between 10 and 11 kpc}",
      journal = {A\&A},
     keywords = {stars: abundances, Galaxy: abundances, Galaxy: evolution, stars: variables: cepheids},
         year = 2004,
        month = jan,
       volume = {413},
        pages = {159-172},
          doi = {10.1051/0004-6361:20031528},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...413..159A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Lepine_etal2014,
       author = {{L{\'e}pine}, Jacques R.~D. and {Andrievky}, Sergei and
         {Barros}, Douglas A. and {Junqueira}, Thiago C. and {Scarano}, Sergio},
        title = "{Bimodal chemical evolution of the Galactic disk and the Barium abundance of Cepheids}",
     keywords = {Galaxy: abundances, Galaxy: evolution, galaxies: spiral, stellar dynamics, stars: Cepheids, Astrophysics - Astrophysics of Galaxies},
    booktitle = {Setting the scene for Gaia and LAMOST},
         year = 2014,
       editor = {{Feltzing}, Sofia and {Zhao}, Gang and {Walton}, Nicholas A. and
         {Whitelock}, Patricia},
       volume = {298},
        month = jan,
        pages = {86-91},
          doi = {10.1017/S174392131300625X},
archivePrefix = {arXiv},
       eprint = {1307.7781},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014IAUS..298...86L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Scarano_Lepine2013,
       author = {{Scarano}, S. and {L{\'e}pine}, J.~R.~D.},
        title = "{Radial metallicity distribution breaks at corotation radius in spiral galaxies}",
      journal = {MNRAS},
     keywords = {galaxies: abundances, galaxies: fundamental parameters, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = jan,
       volume = {428},
       number = {1},
        pages = {625-640},
          doi = {10.1093/mnras/sts048},
archivePrefix = {arXiv},
       eprint = {1209.5031},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.428..625S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amores_etal2009,
       author = {{Am{\^o}res}, E.~B. and {L{\'e}pine}, J.~R.~D. and {Mishurov}, Yu. N.},
        title = "{The corotation gap in the Galactic HI distribution}",
      journal = {MNRAS},
     keywords = {Galaxy: disc, Galaxy: general, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: spiral, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = dec,
       volume = {400},
       number = {4},
        pages = {1768-1774},
          doi = {10.1111/j.1365-2966.2009.15611.x},
archivePrefix = {arXiv},
       eprint = {0907.4822},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.400.1768A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mishurov2000,
       author = {{Mishurov}, Yu. N.},
        title = "{The Gap in the Gaseous Disk of the Galaxy as a Manifestation of Processes in the Corotation Region}",
      journal = {Astronomy Reports},
         year = 2000,
        month = jan,
       volume = {44},
       number = {1},
        pages = {6-11},
          doi = {10.1134/1.163825},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ARep...44....6M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine_etal2001,
       author = {{L{\'e}pine}, J.~R.~D. and {Mishurov}, Yu. N. and {Dedikov}, S. Yu.},
        title = "{A New Model for the Spiral Structure of the Galaxy: Superposition of 2- and 4-armed Patterns}",
      journal = {ApJ},
     keywords = {Galaxy: Kinematics and Dynamics, Galaxy: Structure, Astrophysics},
         year = 2001,
        month = jan,
       volume = {546},
       number = {1},
        pages = {234-247},
          doi = {10.1086/318225},
archivePrefix = {arXiv},
       eprint = {astro-ph/0001216},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...546..234L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalberla_etal2005,
       author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, Dap and
         {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and
         {P{\"o}ppel}, W.~G.~L.},
        title = "{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}",
      journal = {A\&A},
     keywords = {surveys, radio lines: ISM, Galaxy: structure, Astrophysics},
         year = 2005,
        month = sep,
       volume = {440},
       number = {2},
        pages = {775-782},
          doi = {10.1051/0004-6361:20041864},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504140},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...440..775K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lacey_Fall1985,
       author = {{Lacey}, C.~G. and {Fall}, S.~M.},
        title = "{Chemical evolution of the galactic disk with radial gas flows.}",
      journal = {ApJ},
     keywords = {Cosmochemistry, Galactic Evolution, Interstellar Gas, Milky Way Galaxy, Abundance, Gas Flow, Radial Flow, Star Formation Rate, Stellar Evolution, Stellar Structure, Astrophysics},
         year = 1985,
        month = mar,
       volume = {290},
        pages = {154-170},
          doi = {10.1086/162970},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...290..154L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barros_etal2013,
       author = {{Barros}, D.~A. and {L{\'e}pine}, J.~R.~D. and {Junqueira}, T.~C.},
        title = "{A Galactic ring of minimum stellar density near the solar orbit radius}",
      journal = {MNRAS},
     keywords = {stars: kinematics and dynamics, Galaxy: evolution, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {435},
       number = {3},
        pages = {2299-2321},
          doi = {10.1093/mnras/stt1454},
archivePrefix = {arXiv},
       eprint = {1308.0627},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.2299B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bailer-Jones2009,
       author = {{Bailer-Jones}, C.~A.~L.},
        title = "{The evidence for and against astronomical impacts on climate change and mass extinctions: a review}",
      journal = {International Journal of Astrobiology},
     keywords = {climate change, cosmic rays, hypothesis testing, mass extinctions, minor body impacts, period detection, solar motion, spiral arms, time series analysis, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Physics - Geophysics, Quantitative Biology - Populations and Evolution},
         year = 2009,
        month = jul,
       volume = {8},
       number = {3},
        pages = {213-219},
          doi = {10.1017/S147355040999005X},
archivePrefix = {arXiv},
       eprint = {0905.3919},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009IJAsB...8..213B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dias_etal2019,
       author = {{Dias}, W.~S. and {Monteiro}, H. and {L{\'e}pine}, J.~R.~D. and
         {Barros}, D.~A.},
        title = "{The spiral pattern rotation speed of the Galaxy and the corotation radius with Gaia DR2}",
      journal = {MNRAS},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jul,
       volume = {486},
       number = {4},
        pages = {5726-5736},
          doi = {10.1093/mnras/stz1196},
archivePrefix = {arXiv},
       eprint = {1905.08133},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.5726D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gerhard2011,
       author = {{Gerhard}, O.},
        title = "{Pattern speeds in the Milky Way.}",
      journal = {Memorie della Societa Astronomica Italiana Supplementi},
     keywords = {Galaxy: structure, Galaxy: kinematics and dynamics, Galaxy: fundamental parameters, Galaxy: disk, Galaxy: bulge, Galaxies: spiral, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2011,
        month = jan,
       volume = {18},
        pages = {185},
archivePrefix = {arXiv},
       eprint = {1003.2489},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MSAIS..18..185G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marochnik1972,
   author = {{Marochnik}, L.~S. and {Mishurov}, Y.~N. and {Suchkov}, A.~A.
	},
    title = "{On the Spiral Structure of our Galaxy}",
  journal = {ApSS},
     year = 1972,
    month = dec,
   volume = 19,
    pages = {285-292},
      doi = {10.1007/BF00645713},
   adsurl = {http://adsabs.harvard.edu/abs/1972Ap%26SS..19..285M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Creze_Mennessier1973,
   author = {{Creze}, M. and {Mennessier}, M.~O.},
    title = "{An Attempt to Interpret the Mean Properties of the Velocity Field of Young Stars in Terms of Lin's Theory of Spiral Waves}",
  journal = {A\&A},
     year = 1973,
    month = sep,
   volume = 27,
    pages = {281},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....27..281C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mishurov_Zenina1999,
   author = {{Mishurov}, Y.~N. and {Zenina}, I.~A.},
    title = "{Yes, the Sun is located near the corotation circle}",
  journal = {A\&A},
 keywords = {GALAXY: KINEMATICS AND DYNAMICS, GALAXY: STRUCTURE},
     year = 1999,
    month = jan,
   volume = 341,
    pages = {81-85},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...341...81M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marochnik1983b,
       author = {{Marochnik}, L.~S.},
        title = "{On the position of the Sun in the Galaxy}",
      journal = {Astrophysics},
         year = 1983,
        month = jul,
       volume = {19},
       number = {3},
        pages = {278-283},
          doi = {10.1007/BF01007342},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983Ap.....19..278M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marochnik1983a,
       author = {{Marochnik}, L.~S.},
        title = "{On the Origin of the Solar System and the Exceptional Position of the Sun in the Galaxy}",
      journal = {ApSS},
     keywords = {Cosmology, Galactic Structure, Milky Way Galaxy, Solar System, Sun, Angular Momentum, Density Wave Model, Galactic Rotation, Spiral Galaxies, Stellar Evolution, Astrophysics},
         year = 1983,
        month = jan,
       volume = {89},
       number = {1},
        pages = {61-75},
          doi = {10.1007/BF01008385},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983Ap&SS..89...61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dias_Lepine2005,
   author = {{Dias}, W.~S. and {L{\'e}pine}, J.~R.~D.},
    title = "{Direct Determination of the Spiral Pattern Rotation Speed of the Galaxy}",
  journal = {ApJ},
   eprint = {arXiv:astro-ph/0503083},
 keywords = {Galaxy: Disk, Galaxy: Kinematics and Dynamics},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {825-831},
      doi = {10.1086/431456},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..825D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sellwood2011,
   author = {{Sellwood}, J.~A.},
    title = "{The lifetimes of spiral patterns in disc galaxies}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1008.2737},
 primaryClass = "astro-ph.CO",
 keywords = {instabilities, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: spiral},
     year = 2011,
    month = jan,
   volume = 410,
    pages = {1637-1646},
      doi = {10.1111/j.1365-2966.2010.17545.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.410.1637S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Elmegreen_Thomasson1993,
       author = {{Elmegreen}, B.~G. and {Thomasson}, M.},
        title = "{Grand design and flocculent spiral structure in computer simulations with star formation and gas heating.}",
      journal = {A\&A},
         year = 1993,
        month = may,
       volume = {272},
        pages = {37-58},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993A&A...272...37E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang1996,
   author = {{Zhang}, X.},
    title = "{Secular Evolution of Spiral Galaxies. I. A Collective Dissipation Process}",
  journal = {ApJ},
 keywords = {GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: EVOLUTION, GALAXIES: SPIRAL, GALAXIES: STRUCTURE, GALAXY: STRUCTURE, WAVES},
     year = 1996,
    month = jan,
   volume = 457,
    pages = {125 (Z96)},
      doi = {10.1086/176717},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...457..125Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DOnghia_etal2013,
       author = {{D'Onghia}, Elena and {Vogelsberger}, Mark and {Hernquist}, Lars},
        title = "{Self-perpetuating Spiral Arms in Disk Galaxies}",
      journal = {ApJ},
     keywords = {galaxies: kinematics and dynamics, galaxies: spiral, methods: numerical, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = mar,
       volume = {766},
       number = {1},
          eid = {34},
        pages = {34},
          doi = {10.1088/0004-637X/766/1/34},
archivePrefix = {arXiv},
       eprint = {1204.0513},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...766...34D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saha_Elmegreen2016,
       author = {{Saha}, Kanak and {Elmegreen}, Bruce},
        title = "{Long-lived Spiral Structure for Galaxies with Intermediate-size Bulges}",
      journal = {ApJL},
     keywords = {galaxies: bulges, galaxies: evolution, galaxies: halos, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = aug,
       volume = {826},
       number = {2},
          eid = {L21},
        pages = {L21},
          doi = {10.3847/2041-8205/826/2/L21},
archivePrefix = {arXiv},
       eprint = {1607.01953},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826L..21S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fujii_etal2011,
       author = {{Fujii}, M.~S. and {Baba}, J. and {Saitoh}, T.~R. and {Makino}, J. and
         {Kokubo}, E. and {Wada}, K.},
        title = "{The Dynamics of Spiral Arms in Pure Stellar Disks}",
      journal = {ApJ},
     keywords = {galaxies: kinematics and dynamics, galaxies: spiral, methods: numerical, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = apr,
       volume = {730},
       number = {2},
          eid = {109},
        pages = {109},
          doi = {10.1088/0004-637X/730/2/109},
archivePrefix = {arXiv},
       eprint = {1006.1228},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...730..109F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martinez-Garcia_Gonzalez-Lopezlira2013,
       author = {{Mart{\'\i}nez-Garc{\'\i}a}, Eric E. and
         {Gonz{\'a}lez-L{\'o}pezlira}, Rosa A.},
        title = "{Signatures of Long-lived Spiral Patterns}",
      journal = {ApJ},
     keywords = {galaxies: kinematics and dynamics, galaxies: photometry, galaxies: spiral, galaxies: stellar content, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = mar,
       volume = {765},
       number = {2},
          eid = {105},
        pages = {105},
          doi = {10.1088/0004-637X/765/2/105},
archivePrefix = {arXiv},
       eprint = {1301.6634},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...765..105M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pichardo_etal2004,
       author = {{Pichardo}, B{\'a}rbara and {Martos}, Marco and {Moreno}, Edmundo},
        title = "{Models for the Gravitational Field of the Galactic Bar: An Application to Stellar Orbits in the Galactic Plane and Orbits of Some Globular Clusters}",
      journal = {ApJ},
     keywords = {Galaxies: Kinematics and Dynamics, Galaxy: Structure, Galaxy: Globular Clusters: General, Stellar Dynamics, Astrophysics},
         year = 2004,
        month = jul,
       volume = {609},
       number = {1},
        pages = {144-165},
          doi = {10.1086/421008},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402340},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...609..144P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bobylev_etal2014,
       author = {{Bobylev}, V.~V. and {Mosenkov}, A.~V. and {Bajkova}, A.~T. and
         {Gontcharov}, G.~A.},
        title = "{Investigation of the Galactic bar based on photometry and stellar proper motions}",
      journal = {Astronomy Letters},
     keywords = {Galactic structure, central bar, spiral structure, red giant clump, red giant branch stars, stellar proper motions, Astrophysics - Galaxy Astrophysics},
         year = 2014,
        month = feb,
       volume = {40},
       number = {2-3},
        pages = {86-94},
          doi = {10.1134/S1063773714030037},
archivePrefix = {arXiv},
       eprint = {1402.3153},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AstL...40...86B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Portail_etal2017,
       author = {{Portail}, Matthieu and {Gerhard}, Ortwin and {Wegg}, Christopher and
         {Ness}, Melissa},
        title = "{Dynamical modelling of the galactic bulge and bar: the Milky Way's pattern speed, stellar and dark matter mass distribution}",
      journal = {MNRAS},
     keywords = {methods: numerical, Galaxy: bulge, Galaxy: centre, Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = feb,
       volume = {465},
       number = {2},
        pages = {1621-1644},
          doi = {10.1093/mnras/stw2819},
archivePrefix = {arXiv},
       eprint = {1608.07954},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.1621P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rodriguez-Fernandez_Combes2008,
   author = {{Rodriguez-Fernandez}, N.~J. and {Combes}, F.},
    title = "{Gas flow models in the Milky Way embedded bars}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {0806.4252},
 keywords = {Galaxy: structure, Galaxy: center, Galaxy: kinematics and dynamics, ISM: kinematics and dynamics, methods: numerical},
     year = 2008,
    month = oct,
   volume = 489,
    pages = {115-133},
      doi = {10.1051/0004-6361:200809644},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489..115R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sormani_etal2015,
       author = {{Sormani}, Mattia C. and {Binney}, James and {Magorrian}, John},
        title = "{Gas flow in barred potentials - III. Effects of varying the quadrupole}",
      journal = {MNRAS},
     keywords = {ISM: kinematics and dynamics, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = dec,
       volume = {454},
       number = {2},
        pages = {1818-1839},
          doi = {10.1093/mnras/stv2067},
archivePrefix = {arXiv},
       eprint = {1507.03078},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.454.1818S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wegg_etal2015,
       author = {{Wegg}, Christopher and {Gerhard}, Ortwin and {Portail}, Matthieu},
        title = "{The structure of the Milky Way's bar outside the bulge}",
      journal = {MNRAS},
     keywords = {Galaxy: bulge, Galaxy: centre, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {450},
       number = {4},
        pages = {4050-4069},
          doi = {10.1093/mnras/stv745},
archivePrefix = {arXiv},
       eprint = {1504.01401},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.4050W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sormani_etal2015b,
       author = {{Sormani}, Mattia C. and {Binney}, James and {Magorrian}, John},
        title = "{Gas flow in barred potentials - II. Bar-driven spiral arms}",
      journal = {MNRAS},
     keywords = {ISM: kinematics and dynamics, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {451},
       number = {4},
        pages = {3437-3452},
          doi = {10.1093/mnras/stv1135},
archivePrefix = {arXiv},
       eprint = {1504.04807},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.3437S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid_etal2019,
       author = {{Reid}, M.~J. and {Menten}, K.~M. and {Brunthaler}, A. and
         {Zheng}, X.~W. and {Dame}, T.~M. and {Xu}, Y. and {Li}, J. and
         {Sakai}, N. and {Wu}, Y. and {Immer}, K. and {Zhang}, B. and
         {Sanna}, A. and {Moscadelli}, L. and {Rygl}, K.~L.~J. and
         {Bartkiewicz}, A. and {Hu}, B. and {Quiroga-Nu{\~n}ez}, L.~H. and
         {van Langevelde}, H.~J.},
        title = "{Trigonometric Parallaxes of High-mass Star-forming Regions: Our View of the Milky Way}",
      journal = {ApJ},
     keywords = {Milky Way, Milky Way dynamics, Milky Way rotation, Trigonometric parallax, Star formation, Gravitational wave sources, 1054, 1051, 1059, 1713, 1569, 677, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {885},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.3847/1538-4357/ab4a11},
archivePrefix = {arXiv},
       eprint = {1910.03357},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...885..131R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Balazs2000,
       author = {{Bal{\'a}zs}, B{\'e}la},
        title = "{SETI and the Galactic Belt of Intelligent Life}",
    booktitle = {Bioastronomy 99},
         year = 2000,
       editor = {{Lemarchand}, Guillermo and {Meech}, Karen},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {213},
        month = jan,
        pages = {441},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ASPC..213..441B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shaviv2003,
       author = {{Shaviv}, Nir J.},
        title = "{The spiral structure of the Milky Way, cosmic rays, and ice age epochs on Earth}",
      journal = {New Astronomy},
     keywords = {Astrophysics},
         year = 2003,
        month = jan,
       volume = {8},
       number = {1},
        pages = {39-77},
          doi = {10.1016/S1384-1076(02)00193-8},
archivePrefix = {arXiv},
       eprint = {astro-ph/0209252},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003NewA....8...39S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Svensmark2012,
       author = {{Svensmark}, Henrik},
        title = "{Evidence of nearby supernovae affecting life on Earth}",
      journal = {MNRAS},
     keywords = {astrobiology, Earth, supernovae: general, cosmic rays, open clusters and associations: general, Galaxy: structure, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics, Physics - Geophysics},
         year = 2012,
        month = jun,
       volume = {423},
       number = {2},
        pages = {1234-1253},
          doi = {10.1111/j.1365-2966.2012.20953.x},
archivePrefix = {arXiv},
       eprint = {1210.2963},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.423.1234S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rohde_Muller2005,
       author = {{Rohde}, Robert A. and {Muller}, Richard A.},
        title = "{Cycles in fossil diversity}",
      journal = {Nature},
         year = 2005,
        month = mar,
       volume = {434},
       number = {7030},
        pages = {208-210},
          doi = {10.1038/nature03339},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005Natur.434..208R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sartori_etal2003,
       author = {{Sartori}, M.~J. and {L{\'e}pine}, J.~R.~D. and {Dias}, W.~S.},
        title = "{Formation scenarios for the young stellar associations between galactic longitudes l = 280degr - 360degr}",
      journal = {A\&A},
     keywords = {stars: formation, stars: pre-main sequence, stars: early-type, stars: kinematics, stars: Hertzsprung-Russell (HR) and C-M diagrams, open clusters and associations: general, Astrophysics},
         year = 2003,
        month = jun,
       volume = {404},
        pages = {913-926},
          doi = {10.1051/0004-6361:20030581},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304426},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...404..913S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lineweaver_etal2004,
       author = {{Lineweaver}, Charles H. and {Fenner}, Yeshe and {Gibson}, Brad K.},
        title = "{The Galactic Habitable Zone and the Age Distribution of Complex Life in the Milky Way}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics},
         year = 2004,
        month = jan,
       volume = {303},
       number = {5654},
        pages = {59-62},
          doi = {10.1126/science.1092322},
archivePrefix = {arXiv},
       eprint = {astro-ph/0401024},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004Sci...303...59L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gonzalez_etal2001,
       author = {{Gonzalez}, Guillermo and {Brownlee}, Donald and {Ward}, Peter},
        title = "{The Galactic Habitable Zone: Galactic Chemical Evolution}",
      journal = {Icarus},
     keywords = {Astrophysics},
         year = 2001,
        month = jul,
       volume = {152},
       number = {1},
        pages = {185-200},
          doi = {10.1006/icar.2001.6617},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103165},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001Icar..152..185G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Filipovic_etal2013,
       author = {{Filipovic}, M.~D. and {Horner}, J. and {Crawford}, E.~J. and
         {Tothill}, N.~F.~H. and {White}, G.~L.},
        title = "{Mass Extinction and the Structure of the Milky Way}",
      journal = {Serbian Astronomical Journal},
     keywords = {galaxy: structure, astrobiology, solar neighbourhood, Astrophysics - Astrophysics of Galaxies, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = dec,
       volume = {187},
        pages = {43-52},
          doi = {10.2298/SAJ130819005F},
archivePrefix = {arXiv},
       eprint = {1309.4838},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013SerAJ.187...43F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perez-Villegas_etal2015,
       author = {{P{\'e}rez-Villegas}, Angeles and {G{\'o}mez}, Gilberto C. and {Pichardo}, B{\'a}rbara},
        title = "{The galactic branches as a possible evidence for transient spiral arms}",
      journal = {MNRAS},
     keywords = {MHD, Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = aug,
       volume = {451},
       number = {3},
        pages = {2922-2932},
          doi = {10.1093/mnras/stv1157},
archivePrefix = {arXiv},
       eprint = {1505.04327},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.2922P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid2009,
       author = {{Reid}, M.~J. and {Menten}, K.~M. and {Zheng}, X.~W. and {Brunthaler}, A. and {Moscadelli}, L. and {Xu}, Y. and {Zhang}, B. and {Sato}, M. and {Honma}, M. and {Hirota}, T. and {Hachisuka}, K. and {Choi}, Y.~K. and {Moellenbrock}, G.~A. and {Bartkiewicz}, A.},
        title = "{Trigonometric Parallaxes of Massive Star-Forming Regions. VI. Galactic Structure, Fundamental Parameters, and Noncircular Motions}",
      journal = {ApJ},
     keywords = {astrometry, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: formation, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {700},
       number = {1},
        pages = {137-148},
          doi = {10.1088/0004-637X/700/1/137},
archivePrefix = {arXiv},
       eprint = {0902.3913},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700..137R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rubinstein1997,
   author = {{Rubinstein}, R.~Y.},
   title = "{Optimization of computer simulation models with rare events.}",
  journal = {European Journal of Operational Research},
     year = 1997,
publisher = {Elsevier},
   volume = 99,
    pages = {89}
}

@ARTICLE{Rubinstein1999,
   author = {{Rubinstein}, R.~Y.},
   title = "{The Cross-Entropy Method for Combinatorial and Continuous Optimization.}",
  journal = {Methodology and Computing in Applied Probability},
     year = 1999,
publisher = {Springer Link},
   volume = 1,
    pages = {127}
}

@ARTICLE{Kroese2006,
   author = {{Kroese}, D.~P. and {Porotsky}, S. and {Rubinstein}, R.~Y.},
   title = "{The Cross-Entropy Method for Continuous Multi-Extremal Optimization.}",
  journal = {Methodology and Computing in Applied Probability},
     year = 2006,
publisher = {Springer Link},
   volume = 8,
    pages = {383}
}

@ARTICLE{Monteiro_Dias_Caetano2010,
   author = {{Monteiro}, H. and {Dias}, W.~S. and {Caetano}, T.~C.},
    title = "{Fitting isochrones to open cluster photometric data. A new global optimization tool}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1003.4230},
 primaryClass = "astro-ph.IM",
 keywords = {open clusters and associations: general, methods: statistical},
     year = 2010,
    month = jun,
   volume = 516,
      eid = {A2},
    pages = {A2},
      doi = {10.1051/0004-6361/200913677},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...516A...2M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dias2014,
   author = {{Dias}, W.~S. and {Monteiro}, H. and {Caetano}, T.~C. and {L{\'e}pine}, J.~R.~D. and 
	{Assafin}, M. and {Oliveira}, A.~F.},
    title = "{Proper motions of the optically visible open clusters based on the UCAC4 catalog}",
  journal = {A\&A},
 keywords = {open clusters and associations: general},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/201323226},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..79D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Drimmel_Poggio2018,
       author = {{Drimmel}, Ronald and {Poggio}, Eloisa},
        title = "{On the Solar Velocity}",
      journal = {Research Notes of the American Astronomical Society},
         year = 2018,
        month = nov,
       volume = {2},
       number = {4},
          eid = {210},
        pages = {210},
          doi = {10.3847/2515-5172/aaef8b},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RNAAS...2..210D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Benjamin2005,
       author = {{Benjamin}, R.~A. and {Churchwell}, E. and {Babler}, B.~L. and {Indebetouw}, R. and {Meade}, M.~R. and {Whitney}, B.~A. and {Watson}, C. and {Wolfire}, M.~G. and {Wolff}, M.~J. and {Ignace}, R. and {Bania}, T.~M. and {Bracker}, S. and {Clemens}, D.~P. and {Chomiuk}, L. and {Cohen}, M. and {Dickey}, J.~M. and {Jackson}, J.~M. and {Kobulnicky}, H.~A. and {Mercer}, E.~P. and {Mathis}, J.~S. and {Stolovy}, S.~R. and {Uzpen}, B.},
        title = "{First GLIMPSE Results on the Stellar Structure of the Galaxy}",
      journal = {ApJL},
     keywords = {Galaxy: Stellar Content, Galaxy: Structure, Infrared: General, Infrared: ISM, Infrared: Stars, ISM: General, Stars: General, Surveys, Astrophysics},
         year = 2005,
        month = sep,
       volume = {630},
       number = {2},
        pages = {L149-L152},
          doi = {10.1086/491785},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508325},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...630L.149B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nishiyama2005,
       author = {{Nishiyama}, Shogo and {Nagata}, Tetsuya and {Baba}, Daisuke and {Haba}, Yasuaki and {Kadowaki}, Ryota and {Kato}, Daisuke and {Kurita}, Mikio and {Nagashima}, Chie and {Nagayama}, Takahiro and {Murai}, Yuka and {Nakajima}, Yasushi and {Tamura}, Motohide and {Nakaya}, Hidehiko and {Sugitani}, Koji and {Naoi}, Takahiro and {Matsunaga}, Noriyuki and {Tanab{\'e}}, Toshihiko and {Kusakabe}, Nobuhiko and {Sato}, Shuji},
        title = "{A Distinct Structure inside the Galactic Bar}",
      journal = {ApJL},
     keywords = {Galaxy: Bulge, Galaxy: Center, Galaxy: Structure, Infrared: Stars, Astrophysics},
         year = 2005,
        month = mar,
       volume = {621},
       number = {2},
        pages = {L105-L108},
          doi = {10.1086/429291},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502058},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...621L.105N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alard2001,
       author = {{Alard}, C.},
        title = "{Another bar in the Bulge}",
      journal = {A\&A},
     keywords = {GALAXY: BULGE, GALAXY: STRUCTURE, Astrophysics},
         year = 2001,
        month = dec,
       volume = {379},
        pages = {L44-L47},
          doi = {10.1051/0004-6361:20011487},
archivePrefix = {arXiv},
       eprint = {astro-ph/0110491},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...379L..44A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McWillian_Zoccali2010,
       author = {{McWilliam}, Andrew and {Zoccali}, Manuela},
        title = "{Two Red Clumps and the X-shaped Milky Way Bulge}",
      journal = {ApJ},
     keywords = {Galaxy: bulge, Galaxy: structure, stars: distances, stars: late-type, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = dec,
       volume = {724},
       number = {2},
        pages = {1491-1502},
          doi = {10.1088/0004-637X/724/2/1491},
archivePrefix = {arXiv},
       eprint = {1008.0519},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...724.1491M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saito2011,
       author = {{Saito}, R.~K. and {Zoccali}, M. and {McWilliam}, A. and {Minniti}, D. and {Gonzalez}, O.~A. and {Hill}, V.},
        title = "{Mapping the X-shaped Milky Way Bulge}",
      journal = {AJ},
     keywords = {Galaxy: bulge, Galaxy: structure, stars: distances, stars: late-type, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = sep,
       volume = {142},
       number = {3},
          eid = {76},
        pages = {76},
          doi = {10.1088/0004-6256/142/3/76},
archivePrefix = {arXiv},
       eprint = {1107.5360},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142...76S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wegg_Gerhard2013,
       author = {{Wegg}, Christopher and {Gerhard}, Ortwin},
        title = "{Mapping the three-dimensional density of the Galactic bulge with VVV red clump stars}",
      journal = {MNRAS},
     keywords = {Galaxy: bulge, Galaxy: centre, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {435},
       number = {3},
        pages = {1874-1887},
          doi = {10.1093/mnras/stt1376},
archivePrefix = {arXiv},
       eprint = {1308.0593},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.1874W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Michtchenko2019,
       author = {{Michtchenko}, Tatiana A. and {Barros}, Douglas A. and {P{\'e}rez-Villegas}, Angeles and {L{\'e}pine}, Jacques R.~D.},
        title = "{Moving Groups as the Origin of the Vertical Phase Space Spiral in the Solar Neighborhood}",
      journal = {ApJ},
     keywords = {galaxies: spiral, Galaxy: kinematics and dynamics, Galaxy: structure, solar neighborhood},
         year = 2019,
        month = may,
       volume = {876},
       number = {1},
          eid = {36},
        pages = {36},
          doi = {10.3847/1538-4357/ab11cd},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...876...36M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spinelli2021,
       author = {{Spinelli}, R. and {Ghirlanda}, G. and {Haardt}, F. and {Ghisellini}, G. and {Scuderi}, G.},
        title = "{The best place and time to live in the Milky Way}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = sep,
          eid = {arXiv:2009.13539},
        pages = {arXiv:2009.13539},
archivePrefix = {arXiv},
       eprint = {2009.13539},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200913539S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gonzalez2001,
       author = {{Gonzalez}, Guillermo and {Brownlee}, Donald and {Ward}, Peter},
        title = "{The Galactic Habitable Zone: Galactic Chemical Evolution}",
      journal = {Icarus},
     keywords = {Astrophysics},
         year = 2001,
        month = jul,
       volume = {152},
       number = {1},
        pages = {185-200},
          doi = {10.1006/icar.2001.6617},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103165},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001Icar..152..185G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clark1977,
       author = {{Clark}, D.~H. and {McCrea}, W.~H. and {Stephenson}, F.~R.},
        title = "{Frequency of nearby supernovae and climatic and biological catastrophes}",
      journal = {Nature},
     keywords = {Catastrophe Theory, Climatology, Interstellar Matter, Supernovae, Astronomical Models, Ice Formation, Solar System, Space Radiation},
         year = 1977,
        month = jan,
       volume = {265},
       number = {5592},
        pages = {318-319},
          doi = {10.1038/265318a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977Natur.265..318C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


